Finer-CAM: Spotting the Difference Reveals Finer Details for Visual Explanation

Class activation map (CAM) has been widely used to highlight image regions that contribute to class predictions. Despite its simplicity and computational efficiency, CAM often struggles to identify discriminative regions that distinguish visually similar fine-grained classes. Prior efforts address this limitation by introducing more sophisticated explanation processes, but at the cost of extra complexity. In this paper, we propose Finer-CAM, a method that retains CAM's efficiency while achieving precise localization of discriminative regions. Our key insight is that the deficiency of CAM lies not in "how" it explains, but in "what" it explains. Specifically, previous methods attempt to identify all cues contributing to the target class's logit value, which inadvertently also activates regions predictive of visually similar classes. By explicitly comparing the target class with similar classes and spotting their differences, Finer-CAM suppresses features shared with other classes and emphasizes the unique, discriminative details of the target class. Finer-CAM is easy to implement, compatible with various CAM methods, and can be extended to multi-modal models for accurate localization of specific concepts. Additionally, Finer-CAM allows adjustable comparison strength, enabling users to selectively highlight coarse object contours or fine discriminative details. Quantitatively, we show that masking out the top 5% of activated pixels by Finer-CAM results in a larger relative confidence drop compared to baselines. The source code and demo are available at https://github.com/Imageomics/Finer-CAM.

==> tables/rbt_comp.tex <==

\begin{table}[h]
    \centering
    \scriptsize
    \setlength{\tabcolsep}{2pt} 
    % \resizebox{1\linewidth}{!}{ % Resize table
    \vspace{-6pt}
    \begin{tabular}{l|ccc|ccc}
    \toprule
        \multirow{2}{*}{Method} & \multicolumn{3}{c|}{CUB} & \multicolumn{3}{c}{Cars} \\
        & RD.$_{\text{@}0.05}$ $\uparrow$ & RD.$_{\text{@}0.1}$ $\uparrow$ & Loc. $\uparrow$ & RD.$_{\text{@}0.05}$ $\uparrow$ & RD.$_{\text{@}0.1}$ $\uparrow$ & Loc. $\uparrow$ \\
    \midrule
        EVET-Grad &
        0.086 & 0.102 & 0.588 &
        0.055 & 0.067 & 0.559 \\
        SHAP &
        0.099 & 0.103  &  0.493 &  0.054 & 0.065  & 0.504 \\

        % Finer-Grad$^w$ &
        % 0.098 & 0.111  & 0.603 & \textbf{0.060} &\textbf{0.072} & 0.562  \\
        Finer-Grad &
        \textbf{0.112} &\textbf{0.121} & \textbf{0.629} &
        \textbf{0.060} & \textbf{0.071} & \textbf{0.565} \\
    \bottomrule
    \end{tabular}
    % }
\vspace{-6pt}
    \caption{Quantitative comparison with EVET and SHAP.}
    \label{tab:rbt-comp}
\vspace{-10pt}
\end{table}

% \begin{table}[h]
%     \centering
%     \scriptsize
%     \setlength{\tabcolsep}{2pt} 
%     \resizebox{1\linewidth}{!}{ % Resize table
%     \begin{tabular}{l|cccc|cccc}
%     \toprule
%         \multirow{2}{*}{Method} & \multicolumn{4}{c|}{CUB} & \multicolumn{4}{c}{Cars} \\
%         & Del. $\downarrow$ & RD.$_{\text{@}0.05}$ $\uparrow$ & RD.$_{\text{@}0.1}$ $\uparrow$ & Loc. $\uparrow$ & Del. $\downarrow$ & RD.$_{\text{@}0.05}$ $\uparrow$ & RD.$_{\text{@}0.1}$ $\uparrow$ & Loc. $\uparrow$ \\
%     \midrule
%         EVET-Grad &
%         0.028& 0.086 & 0.102 & 0.588 &
%         0.024& 0.055 & 0.067& 0.559 \\
%         SHAP &
%         0.025 &0.099  &0.103  &  0.493&
%         \textbf{0.023} &  0.054& 0.065  & 0.504 \\

%         Finer-Grad$^w$ &
%         0.033& 0.098 &0.111  & 0.603 &
%         0.027& \textbf{0.060} &\textbf{0.072} & 0.562  \\
%         Finer-Grad &
%         \textbf{0.024} & \textbf{0.121} &\textbf{0.121} & \textbf{0.629}&
%         0.024 &\textbf{0.060}  & 0.071 & \textbf{0.565} \\
%     \bottomrule
%     \end{tabular}}
% \vspace{-4pt}
%     \caption{}
%     \label{tab:rbt-comp}
% \vspace{-6pt}
% \end{table}


==> tables/rbt_edge.tex <==

\iffalse
\begin{table}[h]
    \centering
    \scriptsize
    \setlength{\tabcolsep}{2pt} 
    % \resizebox{1\linewidth}{!}{ % Resize table
    \vspace{-6pt}
    \begin{tabular}{l|ccc|ccc}
    \toprule
        \multirow{2}{*}{Method} & \multicolumn{3}{c|}{Confident} & \multicolumn{3}{c}{Confused} \\
        & RD.$_{\text{@}0.05}$ $\uparrow$ & RD.$_{\text{@}0.1}$ $\uparrow$ & Loc. $\uparrow$ & RD.$_{\text{@}0.05}$ $\uparrow$ & RD.$_{\text{@}0.1}$ $\uparrow$ & Loc. $\uparrow$ \\
    \midrule
        % Grad &  0.336& 0.489 &  0.640
        % &  0.005 &0.002 & 0.545\\
        Finer-Grad$^w$  & 0.329 & 0.464 & 0.647
        & \textbf{0.014}&\textbf{0.010}& \textbf{0.600} \\
        Finer-Grad & \textbf{0.349}& \textbf{0.501} &\textbf{0.662}
        &0.008 & 0.005  & 0.598 \\
    \bottomrule
    \end{tabular}
    % }
\vspace{-6pt}
    \caption{Comparison with the weighted average for edge cases.}
    \label{tab:rbt-edge}
\vspace{-10pt}
\end{table}
\fi


% \begin{table}[h]
%     \centering
%     \scriptsize
%     \setlength{\tabcolsep}{2pt} 
%     \resizebox{1\linewidth}{!}{ % Resize table
%     \begin{tabular}{l|cccc|cccc}
%     \toprule
%         \multirow{2}{*}{Method} & \multicolumn{4}{c|}{Confident} & \multicolumn{4}{c}{Confused} \\
%         & Del. $\downarrow$ & RD.$_{\text{@}0.05}$ $\uparrow$ & RD.$_{\text{@}0.1}$ $\uparrow$ & Loc. $\uparrow$ & Del. $\downarrow$ & RD.$_{\text{@}0.05}$ $\uparrow$ & RD.$_{\text{@}0.1}$ $\uparrow$ & Loc. $\uparrow$ \\
%     \midrule
%         Grad &0.106 &  0.336& 0.489 &  0.640
%         &  \textbf{0.012}&  0.005 &0.002 & 0.545\\
%         Finer-Grad &\textbf{0.105 } & \textbf{0.349}& \textbf{0.501} &\textbf{0.662}
%         & \textbf{0.012} &\textbf{ 0.008} &\textbf{0.005}  &\textbf{0.598} \\
%     \bottomrule
%     \end{tabular}}
% \vspace{-4pt}
%     \caption{}
%     \label{tab:rbt-edge}
% \vspace{-12pt}
% \end{table}


==> tables/rbt_ttest.tex <==
\begin{table}[h]
    \centering
    \scriptsize
    \setlength{\tabcolsep}{2pt} 
    % \resizebox{1\linewidth}{!}{ % Resize table
    \vspace{-6pt}
    \begin{tabular}{l|ccc}
    \toprule
        Cars & RD.$_{\text{@}0.05}$ & RD.$_{\text{@}0.1}$ & Loc. \\
    \midrule
        % Grad &  0.336& 0.489 &  0.640
        % &  0.005 &0.002 & 0.545\\
        $t$  & -6.026 & -5.352 & -4.385 \\
        $p$ & 1e-6 & 1e-6 & 1e-5 \\
    \bottomrule
    \end{tabular}
    % }
\vspace{-6pt}
    \caption{Comparison with the weighted average for edge cases.}
    \label{tab:rbt-ttest}
\vspace{-10pt}
\end{table}

